A Rate-Distortion Framework for Explaining Black-box Model Decisions

We present the Rate-Distortion Explanation (RDE) framework, a mathematically well-founded method for explaining black-box model decisions. The framework is based on perturbations of the target input signal and applies to any differentiable pre-trained model such as neural networks. Our experiments demonstrate the framework's adaptability to diverse data modalities, particularly images, audio, and physical simulations of urban environments.

==> Figures/NsynthExplain.tex <==
\begin{figure}[h]
	\centering
	\begin{subfigure}{0.9\textwidth}\centering%no!\hfill
		\includegraphics[width=0.7\linewidth]{Figures/NSynthImages/input_and_sresult11_l50.png}\\
		\label{fig:nsynth_exp1}
	\end{subfigure}%
	
	\begin{subfigure}{0.9\textwidth}\centering
		\includegraphics[width=0.7\linewidth]{Figures/NSynthImages/input_and_sresult31_l50.png}
	   \label{fig:nsynth_exp1}
	\end{subfigure}%
	\caption{\textbf{Radio map estimations}: The output radio map (gray), input buildings (blue), and input measurements (red).}
	\label{fig:radio}
\end{figure}

==> Figures/NsynthExplainability.tex <==
\includegraphics[width=0.7\linewidth]{Figures/NSynthImages/input_and_sresult11_l50.png}\\
\vspace{0.5cm}
\includegraphics[width=0.7\linewidth]{Figures/NSynthImages/input_and_sresult31_l50.png}

==> Tables/MagVsPhaseTable.tex <==
\begin{table}[t]
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{footnotesize}
\begin{sc}
\begin{tabular}{lrr}
\toprule
Intrument & Magnitude & Phase \\
 &  Importance &  Importance\\
\midrule
Organ  & 0.829 & 1.0\\
Guitar & 0.0 & 0.999\\
Flute  & 0.092 & 1.0\\
Bass   & 1.0 & 1.0\\
Reed   & 0.136 & 1.0\\
Vocal  & 1.0 & 1.0\\
Mallet & 0.005   & 0.217\\
Brass  & 0.999 & 1.0\\
Keyboard & 0.003 & 1.0\\
String & 1.0 & 0.0\\
\bottomrule
\end{tabular}
\end{sc}
\end{footnotesize}
\end{center}
\caption{Magnitude Importance vs. Phase Importance.}
\label{tab:mag_vs_phase}
\vskip -0.1in
\end{table}

